Contracting with a Learning Agent

Many real-life contractual relations differ completely from the clean, static model at the heart of principal-agent theory. Typically, they involve repeated strategic interactions of the principal and agent, taking place under uncertainty and over time. While appealing in theory, players seldom use complex dynamic strategies in practice, often preferring to circumvent complexity and approach uncertainty through learning. We initiate the study of repeated contracts with a learning agent, focusing on agents who achieve no-regret outcomes. Optimizing against a no-regret agent is a known open problem in general games; we achieve an optimal solution to this problem for a canonical contract setting, in which the agent's choice among multiple actions leads to success/failure. The solution has a surprisingly simple structure: for some $\alpha > 0$, initially offer the agent a linear contract with scalar $\alpha$, then switch to offering a linear contract with scalar $0$. This switch causes the agent to ``free-fall'' through their action space and during this time provides the principal with non-zero reward at zero cost. Despite apparent exploitation of the agent, this dynamic contract can leave \emph{both} players better off compared to the best static contract. Our results generalize beyond success/failure, to arbitrary non-linear contracts which the principal rescales dynamically. Finally, we quantify the dependence of our results on knowledge of the time horizon, and are the first to address this consideration in the study of strategizing against learning agents.

==> discussion.tex <==



% \paragraph{Smarter Learning}
% \begin{itemize}
%     \item Agents who are learning but also individually rational in the sense that they do not play actions with negative expected utility. \yk{We need to decide how this works, and whether the agents observe the contracts before they play. See the comments above.}
%     \item \yk{A possible model of smarter learners: Consider a meta algorithm with a ``tolerance'' parameter $\tau = o(T)$ that runs any other mean-based learning algorithm, but zeroes-out the accumulated utility of action $a$ if $a$ gave negative average payoff over a window of the last $\tau$ consecutive steps. This should be enough to fix the persistence of mean-based algorithms on bad actions.}  
%     \item \yk{An alternative meta-algorithm: Loss aversion. Play any mean based algorithm but count all negative payoffs as if they are multiplied by a constant $\xi > 1$.}
% \end{itemize}


%% Maybe add to discussion: 
% \subsection{Questions / variations}

% \paragraph{Dynamics with evolving states (last obtained outcome can be the state). E.g., a project with stages, health insurance and investment in health...}

% \paragraph{Agents with types?}

% % \paragraph{MLRP ?}

% \paragraph{Example for a case where free-fall is not optimal?}

% \paragraph{Sufficient conditions for when optimal dynamic contracts improve welfare?}

% \paragraph{Can we characterize the class of contract games where mean-based regret minimization does not do worse (for the agent) in the dynamic setting than the agent's utility under the best static contract? (The agent cannot be exploited.)}








% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection*{Acknowledgments}
%This project has received funding from the European Research Council (ERC) under the European %Union's Horizon 2020 Research and Innovation Programme (grant agreement no. 740282).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
\bibliography{contracts_for_learning_agents_refs}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
% \appendix 
% \newpage
% \section*{Appendix}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> hardness.tex <==

\noindent
\textbf{Hardness}:\\

\noindent
\emph{Conjecture 1}: The problem of finding an optimal free-fall contract for general contract is hard. 
 (And therefore finding an optimal dynamic contract is hard.) Perhaps consider a discrete set of payments? Perhaps similar to TSP?\\

\noindent
\emph{Conjecture 2}: Even with access to an oracle that provides the best free-fall contract, it remains difficult to ascertain whether it is also the optimal dynamic contract in the general case.



==> related.tex <==





%\begin{itemize}
    %\item Strategizing against Learners \cite{BravermanMaoSchneiderWeinberg2018selling},\cite{deng2019strategizing},\\\cite{MansourMohriSchneiderSivan2022strategizing},\cite{cai2023selling}.
    %\item 
    %\item Contracts: \cite{} (Contract Design for Afforestation Programs) \cite{BabaioffKolumbusWinter2022optimal} (Collateral contracts in Investment Networks), \cite{HalacKremerWinter2020raising} (Raising capital from heterogeneous investors)
    %\item Contract dynamics and learning:   \cite{HoSlivkinsWortman2014Adaptive} (Adaptive contract design for crowdsourcing markets: Bandit algorithms for repeated principal-agent problems); \cite{zhu2022sample} (The sample complexity of online contract design);
    %\cite{mu2022solving} (Solving Dynamic Principal-Agent Problems with a Rationally Inattentive Principal).
    %\item Recent work on interactions between learning agents (TBD)
    %\item Recent works on Stackelberg games (TBD)
%\end{itemize}

%The problem of optimizing against a learner has been studied in different contexts: repeated auctions, repeated two-player bimatrix games, and more generally Bayesian games. Roughly, the literature has shown two kinds of results: If the learner is willing to apply a relatively sophisticated learning algorithm that is (close to) no swap regret, then the optimizer cannot exploit the learner -- cannot do better than repeating her best strategy in the one-shot Stackelberg version of the game in which she is the first mover. If however the learner applies a standard no regret algorithm like EXP3, MW or FTPL -- as captured by the large class of \emph{mean-based} learning algorithms -- then the landscape becomes more interesting. 

%In general bimatrix games (not even Bayesian games), optimizing against a mean-based learner is shown to be a variant of a high-dimension control problem -- a solution to which remains an open question. An optimal solution is known for one interesting and well-motivated class of games, namely repeated auctions. For this setting \emph{the entire welfare} can be extracted by the optimal dynamic auction. 
